Sampling-free Uncertainty Estimation in Gated Recurrent Units with Exponential Families

There has recently been a concerted effort to derive mechanisms in vision and machine learning systems to offer uncertainty estimates of the predictions they make. Clearly, there are enormous benefits to a system that is not only accurate but also has a sense for when it is not sure. Existing proposals center around Bayesian interpretations of modern deep architectures -- these are effective but can often be computationally demanding. We show how classical ideas in the literature on exponential families on probabilistic networks provide an excellent starting point to derive uncertainty estimates in Gated Recurrent Units (GRU). Our proposal directly quantifies uncertainty deterministically, without the need for costly sampling-based estimation. We demonstrate how our model can be used to quantitatively and qualitatively measure uncertainty in unsupervised image sequence prediction. To our knowledge, this is the first result describing sampling-free uncertainty estimation for powerful sequential models such as GRUs.

==> experiment.tex <==

\begin{figure*}
	\centering
	\captionsetup[subfigure]{justification=centering,farskip=5pt,captionskip=1pt}
	\setlength{\fboxsep}{0pt}
	\begin{minipage}{90pt} \centering
		\includegraphics[width=\textwidth]{trajs/traj_angle.png}
	\end{minipage}
	\begin{minipage}{110pt} \centering
		\includegraphics[width=\textwidth]{trajs/traj_speed0.png} \\
		\includegraphics[width=\textwidth]{trajs/traj_speed1.png}
	\end{minipage}
	\begin{minipage}{110pt} \centering
		\includegraphics[width=\textwidth]{trajs/traj_speed2.png} \\
		\includegraphics[width=\textwidth]{trajs/traj_speed3.png}
	\end{minipage}
	\vspace{-17pt}
\end{figure*}

%\input{fig_angle_var.tex}
%\input{fig_speed_var.tex}
%\input{fig_noise_var.tex}

==> experiment_old.tex <==

\begin{figure*}
	\centering
	\captionsetup[subfigure]{justification=centering,farskip=5pt,captionskip=1pt}
	\setlength{\fboxsep}{0pt}
	\begin{minipage}{90pt} \centering
		\includegraphics[width=\textwidth]{trajs/traj_angle.png}
	\end{minipage}
	\begin{minipage}{110pt} \centering
		\includegraphics[width=\textwidth]{trajs/traj_speed0.png} \\
		\includegraphics[width=\textwidth]{trajs/traj_speed1.png}
	\end{minipage}
	\begin{minipage}{110pt} \centering
		\includegraphics[width=\textwidth]{trajs/traj_speed2.png} \\
		\includegraphics[width=\textwidth]{trajs/traj_speed3.png}
	\end{minipage}
	\vspace{-17pt}
\end{figure*}

\input{fig_angle_var.tex}
\input{fig_speed_var.tex}
\input{fig_noise_var.tex}
\begin{figure*}
	\centering
	\captionsetup[subfigure]{justification=centering,farskip=5pt,captionskip=1pt}
	\setlength{\fboxsep}{0pt}
		\begin{minipage}{90pt} \centering
			\includegraphics[width=\textwidth]{trajs/traj_angle.png}
		\end{minipage}
		\begin{minipage}{110pt} \centering
			\includegraphics[width=\textwidth]{trajs/traj_speed0.png} \\
			\includegraphics[width=\textwidth]{trajs/traj_speed1.png}
		\end{minipage}
		\begin{minipage}{110pt} \centering
			\includegraphics[width=\textwidth]{trajs/traj_speed2.png} \\
			\includegraphics[width=\textwidth]{trajs/traj_speed3.png}
		\end{minipage}
	\vspace{-17pt}
\end{figure*}


\begin{figure*}
	\centering
	\captionsetup[subfigure]{justification=centering,farskip=5pt,captionskip=1pt}
	\setlength{\fboxsep}{0pt}
	\begin{minipage}{180pt}
		\begin{minipage}{180pt} \centering
			\hspace{10pt}
			\begin{minipage}{53pt} \centering
				\vspace{2pt}\textsf{\footnotesize Ground Truth} 
			\end{minipage}
			\hspace{-2pt}
			\begin{minipage}{53pt} \centering
				\vspace{2pt}\textsf{\footnotesize Prediction} 
			\end{minipage}
			\hspace{-2pt}
			\begin{minipage}{53pt} \centering
				\vspace{2pt}\textsf{\footnotesize Uncertainty} 
				\vspace{-2pt}
			\end{minipage}
			\hspace{-15pt}
		\end{minipage}\\
		\fcolorbox{c1}{white}{\setlength{\fboxrule}{1pt}
			\begin{minipage}{180pt} \centering
				\hspace{-10pt}
				$20^{\circ}$
				\hspace{-8pt}
				\begin{minipage}{60pt} \centering
					\includegraphics[width=0.9\textwidth]{figs_speed_short/99_2future_train_2.png}
				\end{minipage}
				\hspace{-9pt}
				\begin{minipage}{60pt} \centering 
					\includegraphics[width=0.9\textwidth]{figs_speed_short/99_3mean_train_2.png}
				\end{minipage}
				\hspace{-9pt}
				\begin{minipage}{60pt} \centering
					\includegraphics[width=0.9\textwidth]{figs_speed_short/99_4var_train_2.png}
				\end{minipage}
				\hspace{-15pt}
			\end{minipage}
		}\\
		\fcolorbox{c1}{white}{\setlength{\fboxrule}{1pt}
			\begin{minipage}{180pt} \centering
				\hspace{-10pt}
				$25^{\circ}$
				\hspace{-8pt}
				\begin{minipage}{60pt} \centering
					\includegraphics[width=0.9\textwidth]{figs_speed_short/99_2future_test1_2.png}
				\end{minipage}
				\hspace{-9pt}
				\begin{minipage}{60pt} \centering 
					\includegraphics[width=0.9\textwidth]{figs_speed_short/99_3mean_test1_2.png}
				\end{minipage}
				\hspace{-9pt}
				\begin{minipage}{60pt} \centering
					\includegraphics[width=0.9\textwidth]{figs_speed_short/99_4var_test1_2.png}
				\end{minipage}
				\hspace{-15pt}
			\end{minipage}
		}\\
		\fcolorbox{c2}{white}{\setlength{\fboxrule}{1pt}
			\begin{minipage}{180pt} \centering
				\hspace{-10pt}
				$30^{\circ}$
				\hspace{-8pt}
				\begin{minipage}{60pt} \centering
					\includegraphics[width=0.9\textwidth]{figs_speed_short/99_2future_test2_2.png}
				\end{minipage}
				\hspace{-9pt}
				\begin{minipage}{60pt} \centering 
					\includegraphics[width=0.9\textwidth]{figs_speed_short/99_3mean_test2_2.png}
				\end{minipage}
				\hspace{-9pt}
				\begin{minipage}{60pt} \centering
					\includegraphics[width=0.9\textwidth]{figs_speed_short/99_4var_test2_2.png}
				\end{minipage}
				\hspace{-15pt}
			\end{minipage}
		}\\
		\fcolorbox{c3}{white}{\setlength{\fboxrule}{1pt}
			\begin{minipage}{180pt} \centering
				\hspace{-10pt}
				$35^{\circ}$
				\hspace{-8pt}
				\begin{minipage}{60pt} \centering
					\includegraphics[width=0.9\textwidth]{figs_speed_short/99_2future_test3_2.png}
				\end{minipage}
				\hspace{-9pt}
				\begin{minipage}{60pt} \centering 
					\includegraphics[width=0.9\textwidth]{figs_speed_short/99_3mean_test3_2.png}
				\end{minipage}
				\hspace{-9pt}
				\begin{minipage}{60pt} \centering
					\includegraphics[width=0.9\textwidth]{figs_speed_short/99_4var_test3_2.png}
				\end{minipage}
				\hspace{-15pt}
			\end{minipage}
		}\\
	\end{minipage}
	\hspace{10pt}
	\begin{minipage}{120pt} \centering
		\includegraphics[width=\textwidth]{figs_speed2/avg_var_speed2.png}
	\end{minipage}
	\caption{Angle deviation vs. variance}
\end{figure*}

\begin{figure*}
	\centering
	\captionsetup[subfigure]{justification=centering,farskip=5pt,captionskip=1pt}
	\setlength{\fboxsep}{0pt}
	\fcolorbox{green}{white}{\setlength{\fboxrule}{1pt}
		\begin{minipage}{60pt} \centering
			\vspace{2pt}\textsf{\footnotesize Ground Truth} \vspace{1pt}  \\
			\includegraphics[width=\textwidth]{figs_angle_short/99_2future_train_2.png} \\
			\vspace{1pt}
			\includegraphics[width=\textwidth]{figs_angle_short/99_2future_test1_2.png} \\
			\vspace{1pt}
			\includegraphics[width=\textwidth]{figs_angle_short/99_2future_test2_2.png} \\
			\vspace{1pt}
			\includegraphics[width=\textwidth]{figs_angle_short/99_2future_test3_2.png}
			\vspace{1pt}
			\hspace{-4pt}
		\end{minipage}
	}
	\fcolorbox{orange}{white}{\setlength{\fboxrule}{1pt}
		\begin{minipage}{60pt} \centering
			\vspace{2pt}\textsf{\footnotesize Prediction} \vspace{1pt} \\
			\includegraphics[width=\textwidth]{figs_angle_short/99_3mean_train_2.png} \\
			\vspace{1pt}
			\includegraphics[width=\textwidth]{figs_angle_short/99_3mean_test1_2.png} \\
			\vspace{1pt}
			\includegraphics[width=\textwidth]{figs_angle_short/99_3mean_test2_2.png} \\
			\vspace{1pt}
			\includegraphics[width=\textwidth]{figs_angle_short/99_3mean_test3_2.png}
			\vspace{1pt}
			\hspace{-4pt}
		\end{minipage}
	}
	\fcolorbox{magenta}{white}{\setlength{\fboxrule}{1pt}
		\begin{minipage}{60pt} \centering
			\vspace{2pt}\textsf{\footnotesize Uncertainty} \vspace{0pt} \\
			\includegraphics[width=\textwidth]{figs_angle_short/99_4var_train_2.png} \\
			\vspace{1pt}
			\includegraphics[width=\textwidth]{figs_angle_short/99_4var_test1_2.png} \\
			\vspace{1pt}
			\includegraphics[width=\textwidth]{figs_angle_short/99_4var_test2_2.png} \\
			\vspace{1pt}
			\includegraphics[width=\textwidth]{figs_angle_short/99_4var_test3_2.png}
			\vspace{1pt}
			\hspace{-4pt}
		\end{minipage}
	}
	\begin{minipage}{110pt} \centering
		\includegraphics[width=\textwidth]{figs_angle2/avg_var_angle2.png}
	\end{minipage}
	\caption{Angle deviation vs. variance}
\end{figure*}

\begin{figure*}
	\centering
	\captionsetup[subfigure]{justification=centering,farskip=5pt,captionskip=1pt}
	\setlength{\fboxsep}{0pt}
	%	\setlength{\fboxrule}{1pt}
	\fcolorbox{green}{white}{\setlength{\fboxrule}{1pt}
		\begin{minipage}{60pt} \centering
			\vspace{2pt}\textsf{\footnotesize Ground Truth} \vspace{1pt}  \\
			\includegraphics[width=\textwidth]{figs_speed_short/99_2future_train_2.png} \\
			\vspace{1pt}
			\includegraphics[width=\textwidth]{figs_speed_short/99_2future_test1_2.png} \\
			\vspace{1pt}
			\includegraphics[width=\textwidth]{figs_speed_short/99_2future_test2_2.png} \\
			\vspace{1pt}
			\includegraphics[width=\textwidth]{figs_speed_short/99_2future_test3_2.png}
			\vspace{1pt}
			\hspace{-4pt}
		\end{minipage}
	}
	\fcolorbox{orange}{white}{\setlength{\fboxrule}{1pt}
		\begin{minipage}{60pt} \centering
			\vspace{2pt}\textsf{\footnotesize Prediction} \vspace{1pt} \\
			\includegraphics[width=\textwidth]{figs_speed_short/99_3mean_train_2.png} \\
			\vspace{1pt}
			\includegraphics[width=\textwidth]{figs_speed_short/99_3mean_test1_2.png} \\
			\vspace{1pt}
			\includegraphics[width=\textwidth]{figs_speed_short/99_3mean_test2_2.png} \\
			\vspace{1pt}
			\includegraphics[width=\textwidth]{figs_speed_short/99_3mean_test3_2.png}
			\vspace{1pt}
			\hspace{-4pt}
		\end{minipage}
	}
	\fcolorbox{magenta}{white}{\setlength{\fboxrule}{1pt}
		\begin{minipage}{60pt} \centering
			\vspace{2pt}\textsf{\footnotesize Uncertainty} \vspace{0pt} \\
			\includegraphics[width=\textwidth]{figs_speed_short/99_4var_train_2.png} \\
			\vspace{1pt}
			\includegraphics[width=\textwidth]{figs_speed_short/99_4var_test1_2.png} \\
			\vspace{1pt}
			\includegraphics[width=\textwidth]{figs_speed_short/99_4var_test2_2.png} \\
			\vspace{1pt}
			\includegraphics[width=\textwidth]{figs_speed_short/99_4var_test3_2.png}
			\vspace{1pt}
			\hspace{-4pt}
		\end{minipage}
	}
	\begin{minipage}{110pt} \centering
		\includegraphics[width=\textwidth]{figs_speed2/avg_var_speed2.png}
	\end{minipage}
	\caption{Speed deviation vs. variance}
\end{figure*}


\begin{figure*}
	\centering
	\captionsetup[subfigure]{justification=centering,farskip=5pt,captionskip=1pt}
	\setlength{\fboxsep}{0pt}
	%	\setlength{\fboxrule}{1pt}
	\fcolorbox{cyan}{white}{\setlength{\fboxrule}{1pt}
		\begin{minipage}{60pt} \centering
			\vspace{2pt}\textsf{\footnotesize Input} \vspace{0pt}  \\
			\includegraphics[width=\textwidth]{figs_noise_short/99_1input_train_2.png} \\
			\vspace{1pt}
			\includegraphics[width=\textwidth]{figs_noise_short/99_1input_test1_2.png} \\
			\vspace{1pt}
			\includegraphics[width=\textwidth]{figs_noise_short/99_1input_test2_2.png} \\
			\vspace{1pt}
			\includegraphics[width=\textwidth]{figs_noise_short/99_1input_test3_2.png}
			\vspace{1pt}
			\hspace{-4pt}
		\end{minipage}
	}
	\fcolorbox{orange}{white}{\setlength{\fboxrule}{1pt}
		\begin{minipage}{60pt} \centering
			\vspace{2pt}\textsf{\footnotesize Prediction} \vspace{1pt} \\
			\includegraphics[width=\textwidth]{figs_noise_short/99_3mean_train_2.png} \\
			\vspace{1pt}
			\includegraphics[width=\textwidth]{figs_noise_short/99_3mean_test1_2.png} \\
			\vspace{1pt}
			\includegraphics[width=\textwidth]{figs_noise_short/99_3mean_test2_2.png} \\
			\vspace{1pt}
			\includegraphics[width=\textwidth]{figs_noise_short/99_3mean_test3_2.png}
			\vspace{1pt}
			\hspace{-4pt}
		\end{minipage}
	}
	\fcolorbox{magenta}{white}{\setlength{\fboxrule}{1pt}
		\begin{minipage}{60pt} \centering
			\vspace{2pt}\textsf{\footnotesize Uncertainty} \vspace{0pt} \\
			\includegraphics[width=\textwidth]{figs_noise_short/99_4var_train_2.png} \\
			\vspace{1pt}
			\includegraphics[width=\textwidth]{figs_noise_short/99_4var_test1_2.png} \\
			\vspace{1pt}
			\includegraphics[width=\textwidth]{figs_noise_short/99_4var_test2_2.png} \\
			\vspace{1pt}
			\includegraphics[width=\textwidth]{figs_noise_short/99_4var_test3_2.png}
			\vspace{1pt}
			\hspace{-4pt}
		\end{minipage}
	}
	\begin{minipage}{110pt} \centering
		\includegraphics[width=\textwidth]{figs_noise2/avg_var_noise2.png}
	\end{minipage}
	\caption{Pixel-level noise vs. variance}
\end{figure*}
\newpage

%\begin{figure}
%	\includegraphics[width=0.32\textwidth]{figs_angle2/avg_var_angle2.png}
%	\includegraphics[width=0.32\textwidth]{figs_speed2/avg_var_speed2.png}
%	\includegraphics[width=0.32\textwidth]{figs_noise2/avg_var_noise2.png}
%\end{figure}

\begin{figure}
	\includegraphics[width=0.5\textwidth]{figs_angle2/99_1input_train.png}
	\includegraphics[width=0.5\textwidth]{figs_angle2/99_3mean_train.png} \\
	\includegraphics[width=0.5\textwidth]{figs_angle2/99_1input_test1.png}
	\includegraphics[width=0.5\textwidth]{figs_angle2/99_3mean_test1.png} \\
	\includegraphics[width=0.5\textwidth]{figs_angle2/99_1input_test2.png}
	\includegraphics[width=0.5\textwidth]{figs_angle2/99_3mean_test2.png} \\
	\includegraphics[width=0.5\textwidth]{figs_angle2/99_1input_test3.png}
	\includegraphics[width=0.5\textwidth]{figs_angle2/99_3mean_test3.png}
	
	\includegraphics[width=0.8\textwidth]{figs_angle2/avg_var_angle2.png}
\end{figure}

\begin{figure}
	\includegraphics[width=0.5\textwidth]{figs_speed2/99_1input_train.png}
	\includegraphics[width=0.5\textwidth]{figs_speed2/99_3mean_train.png} \\
	\includegraphics[width=0.5\textwidth]{figs_speed2/99_1input_test1.png}
	\includegraphics[width=0.5\textwidth]{figs_speed2/99_3mean_test1.png} \\
	\includegraphics[width=0.5\textwidth]{figs_speed2/99_1input_test2.png}
	\includegraphics[width=0.5\textwidth]{figs_speed2/99_3mean_test2.png} \\
	\includegraphics[width=0.5\textwidth]{figs_speed2/99_1input_test3.png}
	\includegraphics[width=0.5\textwidth]{figs_speed2/99_3mean_test3.png}
	
	\includegraphics[width=0.8\textwidth]{figs_speed2/avg_var_speed2.png}
\end{figure}

\begin{figure}
	\includegraphics[width=0.5\textwidth]{figs_noise2/99_1input_train.png}
	\includegraphics[width=0.5\textwidth]{figs_noise2/99_3mean_train.png} \\
	\includegraphics[width=0.5\textwidth]{figs_noise2/99_1input_test1.png}
	\includegraphics[width=0.5\textwidth]{figs_noise2/99_3mean_test1.png} \\
	\includegraphics[width=0.5\textwidth]{figs_noise2/99_1input_test2.png}
	\includegraphics[width=0.5\textwidth]{figs_noise2/99_3mean_test2.png} \\
	\includegraphics[width=0.5\textwidth]{figs_noise2/99_1input_test3.png}
	\includegraphics[width=0.5\textwidth]{figs_noise2/99_3mean_test3.png}
	
	\includegraphics[width=0.8\textwidth]{figs_noise2/avg_var_noise2.png}
\end{figure}

\begin{figure}
	\includegraphics[width=0.30\textwidth]{trajs/traj_speed0.png} \\
	\includegraphics[width=0.30\textwidth]{trajs/traj_speed1.png} \\
	\includegraphics[width=0.30\textwidth]{trajs/traj_speed2.png} \\
	\includegraphics[width=0.30\textwidth]{trajs/traj_speed3.png}
\end{figure}

==> fig_angle_speed.tex <==
\begin{figure*}
	\centering
	\captionsetup[subfigure]{justification=centering,farskip=5pt,captionskip=1pt}
	\setlength{\fboxsep}{0pt}
	\begin{minipage}{180pt}
		\begin{minipage}{185pt} \centering
			\hspace{2pt}
			\begin{minipage}{6pt} \centering
				\vspace{2pt}\textsf{\footnotesize $v$} 
			\end{minipage}
			\hspace{2pt}
			\begin{minipage}{53pt} \centering
				\vspace{2pt}\textsf{\footnotesize Ground Truth} 
			\end{minipage}
			\hspace{-2pt}
			\begin{minipage}{53pt} \centering
				\vspace{2pt}\textsf{\footnotesize Prediction} 
			\end{minipage}
			\hspace{-2pt}
			\begin{minipage}{53pt} \centering
				\vspace{2pt}\textsf{\footnotesize Uncertainty} 
				\vspace{-2pt}
			\end{minipage}
			\hspace{-15pt}
		\end{minipage}\\
		\fcolorbox{c1}{white}{\setlength{\fboxrule}{1pt}
			\begin{minipage}{185pt} \centering
				\hspace{-10pt}
				{\scriptsize $0.050$}
				\hspace{-8pt}
				\begin{minipage}{60pt} \centering
					\includegraphics[width=0.9\textwidth]{figs_speed_short/99_2future_train_2.png}
				\end{minipage}
				\hspace{-9pt}
				\begin{minipage}{60pt} \centering 
					\includegraphics[width=0.9\textwidth]{figs_speed_short/99_3mean_train_2.png}
				\end{minipage}
				\hspace{-9pt}
				\begin{minipage}{60pt} \centering
					\includegraphics[width=0.9\textwidth]{figs_speed_short/99_4var_train_2.png}
				\end{minipage}
				\hspace{-15pt}
			\end{minipage}
		}\\
		\fcolorbox{c2}{white}{\setlength{\fboxrule}{1pt}
			\begin{minipage}{185pt} \centering
				\hspace{-10pt}
				{\scriptsize $0.055$}
				\hspace{-8pt}
				\begin{minipage}{60pt} \centering
					\includegraphics[width=0.9\textwidth]{figs_speed_short/99_2future_test1_2.png}
				\end{minipage}
				\hspace{-9pt}
				\begin{minipage}{60pt} \centering 
					\includegraphics[width=0.9\textwidth]{figs_speed_short/99_3mean_test1_2.png}
				\end{minipage}
				\hspace{-9pt}
				\begin{minipage}{60pt} \centering
					\includegraphics[width=0.9\textwidth]{figs_speed_short/99_4var_test1_2.png}
				\end{minipage}
				\hspace{-15pt}
			\end{minipage}
		}\\
		\fcolorbox{c3}{white}{\setlength{\fboxrule}{1pt}
			\begin{minipage}{185pt} \centering
				\hspace{-10pt}
				{\scriptsize $0.060$}
				\hspace{-8pt}
				\begin{minipage}{60pt} \centering
					\includegraphics[width=0.9\textwidth]{figs_speed_short/99_2future_test2_2.png}
				\end{minipage}
				\hspace{-9pt}
				\begin{minipage}{60pt} \centering 
					\includegraphics[width=0.9\textwidth]{figs_speed_short/99_3mean_test2_2.png}
				\end{minipage}
				\hspace{-9pt}
				\begin{minipage}{60pt} \centering
					\includegraphics[width=0.9\textwidth]{figs_speed_short/99_4var_test2_2.png}
				\end{minipage}
				\hspace{-15pt}
			\end{minipage}
		}\\
		\fcolorbox{c4}{white}{\setlength{\fboxrule}{1pt}
			\begin{minipage}{185pt} \centering
				\hspace{-10pt}
				{\scriptsize $0.065$}
				\hspace{-8pt}
				\begin{minipage}{60pt} \centering
					\includegraphics[width=0.9\textwidth]{figs_speed_short/99_2future_test3_2.png}
				\end{minipage}
				\hspace{-9pt}
				\begin{minipage}{60pt} \centering 
					\includegraphics[width=0.9\textwidth]{figs_speed_short/99_3mean_test3_2.png}
				\end{minipage}
				\hspace{-9pt}
				\begin{minipage}{60pt} \centering
					\includegraphics[width=0.9\textwidth]{figs_speed_short/99_4var_test3_2.png}
				\end{minipage}
				\hspace{-15pt}
			\end{minipage}
		}\\
	\end{minipage}
	\hspace{10pt}
	\begin{minipage}{120pt} \centering
		\includegraphics[width=\textwidth]{figs_speed2/avg_var_speed2.png}
	\end{minipage}
	\caption{Angle deviation vs. variance}
\end{figure*}


==> fig_angle_var.tex <==
\begin{figure*}[!t]
	\centering
	\captionsetup[subfigure]{justification=centering,farskip=5pt,captionskip=1pt}
	\setlength{\fboxsep}{0pt}
	\begin{minipage}{200pt}
		\begin{minipage}{195pt} \centering
			\hspace{-2pt}
			\begin{minipage}{6pt} \centering
				\vspace{2pt}\textsf{\footnotesize $\theta$} 
			\end{minipage}
			\hspace{2pt}
			\begin{minipage}{53pt} \centering
				\vspace{2pt}\textsf{\footnotesize Ground Truth} 
			\end{minipage}
			\hspace{-2pt}
			\begin{minipage}{53pt} \centering
				\vspace{2pt}\textsf{\footnotesize Prediction} 
			\end{minipage}
			\hspace{-2pt}
			\begin{minipage}{53pt} \centering
				\vspace{2pt}\textsf{\footnotesize Uncertainty} 
				\vspace{-2pt}
			\end{minipage}
			\hspace{-15pt}
		\end{minipage}\\ 
		\fcolorbox{c1}{white}{\setlength{\fboxrule}{1pt}
			\begin{minipage}{190pt} \centering
				\hspace{-10pt}
				$20^{\circ}$
				\hspace{-8pt}
				\begin{minipage}{60pt} \centering
					\includegraphics[width=0.9\textwidth]{figs_angle_short/99_2future_train_2.png}
				\end{minipage}
				\hspace{-9pt}
				\begin{minipage}{60pt} \centering 
					\includegraphics[width=0.9\textwidth]{figs_angle_short/99_3mean_train_2.png}
				\end{minipage}
				\hspace{-9pt}
				\begin{minipage}{60pt} \centering
					\includegraphics[width=0.9\textwidth]{figs_angle_short/99_4var_train_2.png}
				\end{minipage}
				\hspace{-15pt}
			\end{minipage}
		}\\
		\fcolorbox{c2}{white}{\setlength{\fboxrule}{1pt}
			\begin{minipage}{190pt} \centering
				\hspace{-10pt}
				$25^{\circ}$
				\hspace{-8pt}
				\begin{minipage}{60pt} \centering
					\includegraphics[width=0.9\textwidth]{figs_angle_short/99_2future_test1_2.png}
				\end{minipage}
				\hspace{-9pt}
				\begin{minipage}{60pt} \centering 
					\includegraphics[width=0.9\textwidth]{figs_angle_short/99_3mean_test1_2.png}
				\end{minipage}
				\hspace{-9pt}
				\begin{minipage}{60pt} \centering
					\includegraphics[width=0.9\textwidth]{figs_angle_short/99_4var_test1_2.png}
				\end{minipage}
				\hspace{-15pt}
			\end{minipage}
		}\\
		\fcolorbox{c3}{white}{\setlength{\fboxrule}{1pt}
			\begin{minipage}{190pt} \centering
				\hspace{-10pt}
				$30^{\circ}$
				\hspace{-8pt}
				\begin{minipage}{60pt} \centering
					\includegraphics[width=0.9\textwidth]{figs_angle_short/99_2future_test2_2.png}
				\end{minipage}
				\hspace{-9pt}
				\begin{minipage}{60pt} \centering 
					\includegraphics[width=0.9\textwidth]{figs_angle_short/99_3mean_test2_2.png}
				\end{minipage}
				\hspace{-9pt}
				\begin{minipage}{60pt} \centering
					\includegraphics[width=0.9\textwidth]{figs_angle_short/99_4var_test2_2.png}
				\end{minipage}
				\hspace{-15pt}
			\end{minipage}
		}\\
		\fcolorbox{c4}{white}{\setlength{\fboxrule}{1pt}
			\begin{minipage}{190pt} \centering
				\hspace{-10pt}
				$35^{\circ}$
				\hspace{-8pt}
				\begin{minipage}{60pt} \centering
					\includegraphics[width=0.9\textwidth]{figs_angle_short/99_2future_test3_2.png}
				\end{minipage}
				\hspace{-9pt}
				\begin{minipage}{60pt} \centering 
					\includegraphics[width=0.9\textwidth]{figs_angle_short/99_3mean_test3_2.png}
				\end{minipage}
				\hspace{-9pt}
				\begin{minipage}{60pt} \centering
					\includegraphics[width=0.9\textwidth]{figs_angle_short/99_4var_test3_2.png}
				\end{minipage}
				\hspace{-15pt}
			\end{minipage}
		}\\
	\end{minipage}
	\hspace{10pt}
	\begin{minipage}{120pt} \centering
	\vspace{5pt}
		\includegraphics[width=\textwidth]{figs_angle2/sum_var_angle_mc.png}
	\end{minipage}
	\caption{Predictions and uncertainties using a model trained only on $\theta=20$ on varying angles of trajectories (Fig.~\ref{fig:traj}) on a model trained only on $\theta=20$. Right: Average of variance per frame of prediction of SP-GRU and MC-LSTM of 50 samples which both increase as $\theta \uparrow$.}
\end{figure*}


==> fig_noise_var.tex <==
\begin{figure*}[!t]
	\centering
	\captionsetup[subfigure]{justification=centering,farskip=5pt,captionskip=1pt}
	\setlength{\fboxsep}{0pt}
	\begin{minipage}{200pt}
		\begin{minipage}{185pt} \centering
			\hspace{-2pt}
			\begin{minipage}{6pt} \centering
				\vspace{2pt}\textsf{\footnotesize $b$} 
			\end{minipage}
			\hspace{2pt}
			\begin{minipage}{53pt} \centering
				\vspace{2pt}\textsf{\footnotesize Input} 
			\end{minipage}
			\hspace{-2pt}
			\begin{minipage}{53pt} \centering
				\vspace{2pt}\textsf{\footnotesize Prediction} 
			\end{minipage}
			\hspace{-2pt}
			\begin{minipage}{53pt} \centering
				\vspace{2pt}\textsf{\footnotesize Uncertainty} 
				\vspace{-2pt}
			\end{minipage}
			\hspace{-15pt}
		\end{minipage}\\
		\fcolorbox{c1}{white}{\setlength{\fboxrule}{1pt}
			\begin{minipage}{190pt} \centering
				\hspace{-11pt}
				{\scriptsize $0.0$}
				\hspace{-7pt}
				\begin{minipage}{60pt} \centering
					\includegraphics[width=0.9\textwidth]{figs_noise_short/99_1input_train_2.png}
				\end{minipage}
				\hspace{-9pt}
				\begin{minipage}{60pt} \centering 
					\includegraphics[width=0.9\textwidth]{figs_noise_short/99_3mean_train_2.png}
				\end{minipage}
				\hspace{-9pt}
				\begin{minipage}{60pt} \centering
					\includegraphics[width=0.9\textwidth]{figs_noise_short/99_4var_train_2.png}
				\end{minipage}
				\hspace{-15pt}
			\end{minipage}
		}\\
		\fcolorbox{c2}{white}{\setlength{\fboxrule}{1pt}
			\begin{minipage}{190pt} \centering
				\hspace{-11pt}
				{\scriptsize $0.2$}
				\hspace{-7pt}
				\begin{minipage}{60pt} \centering
					\includegraphics[width=0.9\textwidth]{figs_noise_short/99_1input_test1_2.png}
				\end{minipage}
				\hspace{-9pt}
				\begin{minipage}{60pt} \centering 
					\includegraphics[width=0.9\textwidth]{figs_noise_short/99_3mean_test1_2.png}
				\end{minipage}
				\hspace{-9pt}
				\begin{minipage}{60pt} \centering
					\includegraphics[width=0.9\textwidth]{figs_noise_short/99_4var_test1_2.png}
				\end{minipage}
				\hspace{-15pt}
			\end{minipage}
		}\\
		\fcolorbox{c3}{white}{\setlength{\fboxrule}{1pt}
			\begin{minipage}{190pt} \centering
				\hspace{-11pt}
				{\scriptsize $0.4$}
				\hspace{-7pt}
				\begin{minipage}{60pt} \centering
					\includegraphics[width=0.9\textwidth]{figs_noise_short/99_1input_test2_2.png}
				\end{minipage}
				\hspace{-9pt}
				\begin{minipage}{60pt} \centering 
					\includegraphics[width=0.9\textwidth]{figs_noise_short/99_3mean_test2_2.png}
				\end{minipage}
				\hspace{-9pt}
				\begin{minipage}{60pt} \centering
					\includegraphics[width=0.9\textwidth]{figs_noise_short/99_4var_test2_2.png}
				\end{minipage}
				\hspace{-15pt}
			\end{minipage}
		}\\
		\fcolorbox{c4}{white}{\setlength{\fboxrule}{1pt}
			\begin{minipage}{190pt} \centering
				\hspace{-11pt}
				{\scriptsize $0.6$}
				\hspace{-7pt}
				\begin{minipage}{60pt} \centering
					\includegraphics[width=0.9\textwidth]{figs_noise_short/99_1input_test3_2.png}
				\end{minipage}
				\hspace{-9pt}
				\begin{minipage}{60pt} \centering 
					\includegraphics[width=0.9\textwidth]{figs_noise_short/99_3mean_test3_2.png}
				\end{minipage}
				\hspace{-9pt}
				\begin{minipage}{60pt} \centering
					\includegraphics[width=0.9\textwidth]{figs_noise_short/99_4var_test3_2.png}
				\end{minipage}
				\hspace{-15pt}
			\end{minipage}
		}\\
	\end{minipage}
	\hspace{10pt}
	\begin{minipage}{120pt} \centering
		\includegraphics[width=\textwidth]{figs_noise2/sum_var_noise_mc.png}
	\end{minipage}
	\caption{Pixel-wise noise Unif$(0,b)$ vs. variance}
\end{figure*}


==> fig_speed_var.tex <==
\begin{figure*}[!t]
	\centering
	\captionsetup[subfigure]{justification=centering,farskip=5pt,captionskip=1pt}
	\setlength{\fboxsep}{0pt}
	\begin{minipage}{200pt}
		\begin{minipage}{185pt} \centering
			\hspace{-2pt}
			\begin{minipage}{6pt} \centering
				\vspace{2pt}\textsf{\footnotesize $v$} 
			\end{minipage}
			\hspace{2pt}
			\begin{minipage}{53pt} \centering
				\vspace{2pt}\textsf{\footnotesize Ground Truth} 
			\end{minipage}
			\hspace{-2pt}
			\begin{minipage}{53pt} \centering
				\vspace{2pt}\textsf{\footnotesize Prediction} 
			\end{minipage}
			\hspace{-2pt}
			\begin{minipage}{53pt} \centering
				\vspace{2pt}\textsf{\footnotesize Uncertainty} 
				\vspace{-2pt}
			\end{minipage}
			\hspace{-15pt}
		\end{minipage}\\
		\fcolorbox{c1}{white}{\setlength{\fboxrule}{1pt}
			\begin{minipage}{190pt} \centering
				\hspace{-10pt}
				{\scriptsize $5.0$\%}
				\hspace{-8pt}
				\begin{minipage}{60pt} \centering
					\includegraphics[width=0.9\textwidth]{figs_speed_short/99_2future_train_2.png}
				\end{minipage}
				\hspace{-9pt}
				\begin{minipage}{60pt} \centering 
					\includegraphics[width=0.9\textwidth]{figs_speed_short/99_3mean_train_2.png}
				\end{minipage}
				\hspace{-9pt}
				\begin{minipage}{60pt} \centering
					\includegraphics[width=0.9\textwidth]{figs_speed_short/99_4var_train_2.png}
				\end{minipage}
				\hspace{-15pt}
			\end{minipage}
		}\\
		\fcolorbox{c2}{white}{\setlength{\fboxrule}{1pt}
			\begin{minipage}{190pt} \centering
				\hspace{-10pt}
				{\scriptsize  $5.5$\%}
				\hspace{-8pt}
				\begin{minipage}{60pt} \centering
					\includegraphics[width=0.9\textwidth]{figs_speed_short/99_2future_test1_2.png}
				\end{minipage}
				\hspace{-9pt}
				\begin{minipage}{60pt} \centering 
					\includegraphics[width=0.9\textwidth]{figs_speed_short/99_3mean_test1_2.png}
				\end{minipage}
				\hspace{-9pt}
				\begin{minipage}{60pt} \centering
					\includegraphics[width=0.9\textwidth]{figs_speed_short/99_4var_test1_2.png}
				\end{minipage}
				\hspace{-15pt}
			\end{minipage}
		}\\
		\fcolorbox{c3}{white}{\setlength{\fboxrule}{1pt}
			\begin{minipage}{190pt} \centering
				\hspace{-10pt}
				{\scriptsize  $6.0$\%}
				\hspace{-8pt}
				\begin{minipage}{60pt} \centering
					\includegraphics[width=0.9\textwidth]{figs_speed_short/99_2future_test2_2.png}
				\end{minipage}
				\hspace{-9pt}
				\begin{minipage}{60pt} \centering 
					\includegraphics[width=0.9\textwidth]{figs_speed_short/99_3mean_test2_2.png}
				\end{minipage}
				\hspace{-9pt}
				\begin{minipage}{60pt} \centering
					\includegraphics[width=0.9\textwidth]{figs_speed_short/99_4var_test2_2.png}
				\end{minipage}
				\hspace{-15pt}
			\end{minipage}
		}\\
		\fcolorbox{c4}{white}{\setlength{\fboxrule}{1pt}
			\begin{minipage}{190pt} \centering
				\hspace{-10pt}
				{\scriptsize  $6.5$\%}
				\hspace{-8pt}
				\begin{minipage}{60pt} \centering
					\includegraphics[width=0.9\textwidth]{figs_speed_short/99_2future_test3_2.png}
				\end{minipage}
				\hspace{-9pt}
				\begin{minipage}{60pt} \centering 
					\includegraphics[width=0.9\textwidth]{figs_speed_short/99_3mean_test3_2.png}
				\end{minipage}
				\hspace{-9pt}
				\begin{minipage}{60pt} \centering
					\includegraphics[width=0.9\textwidth]{figs_speed_short/99_4var_test3_2.png}
				\end{minipage}
				\hspace{-15pt}
			\end{minipage}
		}\\
	\end{minipage}
	\hspace{10pt}
	\begin{minipage}{120pt} \centering
		\includegraphics[width=\textwidth]{figs_speed2/sum_var_speed_mc.png}
	\end{minipage}
	\caption{Speed deviation $v$ (\% move / frame vs. variance.}
\end{figure*}


==> moreExps.tex <==
\section{Other Methods of Measuring Uncertainty}

Deep Markov Models \cite{krishnan2017structured} introduced recently naturally give rise to a probabilistic interpretation of predictions from deep temporal models. However, upon application of this model to Moving MNIST we were unable to obtain any reasonable prediction, across a range of hidden dimension sizes and trajectory complexities, even with significant training time (days vs. hours for \GRUNAME{}). Shown in Fig. \ref{fig:dmm} are results using a hidden dimension size of 1024, with 100 dimensional hidden state. We note that the experimental setups described in \cite{krishnan2017structured} are small in dimension and complexity compared to Moving MNIST, and it may be the case that small technical development with DMMs may lead to promising and comparable uncertainty results.

\begin{figure}[!h]
	\includegraphics[width=\textwidth]{DMM_result.png}
	\caption{\label{fig:dmm} Results for a single-digit fixed trajectory after 646K iterations using the DMM model. Top: Ground Truth Trajectory. Bottom Right: Predicted trajectory of last 10 frames given first 10. Bottom Left: Uncertainty estimation of predicted trajectory.}
\end{figure}


\subsection{MC-LSTM: Qualitative Comparisons}
In Section 4.1 of the main text, we demonstrated that the uncertainty measures of both SP-GRU and MC-LSTM behave similarly such that the increasing trajectory deviations had also increased the uncertainties (Fig.~7 of main text). However, the absolute magnitudes of these measures do not necessarily translate directly to the quality of uncertainty. For instance, given the same unfamiliar input, if the uncertainty of SP-GRU is higher than that of MC-LSTM, that does not necessarily mean that the uncertainty estimate of SP-GRU is better than that of MC-LSTM. Instead, the relative measure of uncertainty within each model is of more interest which demonstrates how each model appropriately detects the degree of uncertainty given various inputs.

\begin{figure}[h]
	\centering
	\includegraphics[width=0.3\textwidth]{map_ours.png} \hspace{20pt}
	\includegraphics[width=0.3\textwidth]{map_mc.png}
	\caption{\label{fig:map} Uncertainty maps of SP-GRU (left) and MC-LSTM (right) of three identical frames given a trajectory with deviated angle.}
\end{figure}

Thus, in Fig.~\ref{fig:map}, we qualitatively show that the uncertainty measures of the models, despite the small gaps between their quantities, agree with each other. In other words, we see how the uncertainty maps from SP-GRU and MC-LSTM look similar to each other, implying that (1) these models interpret the uncertainty similarly (which is reasonable given the similarity between their basic cell structures) and (2) the between-model uncertainty gaps are of less significance.
